Discovering executable routine specifications from user interaction logs

Robotic Process Automation (RPA) is a technology to automate routine work such as copying data across applications or filling in document templates using data from multiple applications. RPA tools allow organizations to automate a wide range of routines. However, identifying and scoping routines that can be automated using RPA tools is time consuming. Manual identification of candidate routines via interviews, walk-throughs, or job shadowing allow analysts to identify the most visible routines, but these methods are not suitable when it comes to identifying the long tail of routines in an organization. This article proposes an approach to discover automatable routines from logs of user interactions with IT systems and to synthesize executable specifications for such routines. The approach starts by discovering frequent routines at a control-flow level (candidate routines). It then determines which of these candidate routines are automatable and it synthetizes an executable specification for each such routine. Finally, it identifies semantically equivalent routines so as to produce a set of non-redundant automatable routines. The article reports on an evaluation of the approach using a combination of synthetic and real-life logs. The evaluation results show that the approach can discover automatable routines that are known to be present in a UI log, and that it identifies automatable routines that users recognize as such in real-life logs.

==> tables-complete-segmentation.tex <==
\begingroup
%\renewcommand{\arraystretch}{1.6}
\begin{table}[hbtp]
\makebox[0.98\textwidth][c]{
\centering
{\tiny{
    \begin{tabular}{c|c|c|l|l|l|l|l}
    & \textbf{UI}
    & \textbf{UI}
    & \multicolumn{5}{|c}{\textbf{Payload}}
    \\\cline{4-8}

    & \textbf{Timestamp}
    & \textbf{Type}
    & \textbf{\textbf{$P_1$: Application}}
    & \textbf{\textbf{$P_2$: URL}}
    & \textbf{\textbf{$P_3$: Worksheet Name}}
    & \textbf{\textbf{$P_4$: Element Label}}
    & \textbf{\textbf{$P_5$: Cell Column}}\\\hline
    
    \rowcolor{green}
    1 & 2019-03-03T19:02:18 & Click button & Web browser & http://www.unimelb.edu.au & -- & New Record & -- \\\hline
    2 & 2019-03-03T19:02:23 & Copy cell & Worksheet & -- & StudentRecords & -- & A \\\hline 
    3 & 2019-03-03T19:02:26 & Paste & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline 
    4 & 2019-03-03T19:02:28 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline
    5 & 2019-03-03T19:02:31 & Copy cell & Worskheet & -- & StudentRecords & -- & B \\\hline  
    6 & 2019-03-03T19:02:37 & Paste & Web browser & http://www.unimelb.edu.au & -- & Date & -- \\\hline 
    7 & 2019-03-03T19:02:40 & Edit field & Web browser & http://www.unimelb.edu.au &-- & Date & -- \\\hline
    8 & 2019-03-03T19:07:33 & Copy cell & Worksheet & -- & StudentRecords & -- & C \\\hline 
    9 & 2019-03-03T19:07:40 & Paste & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline 
  10 & 2019-03-03T19:07:48 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline
  11 & 2019-03-03T19:07:50 & Copy cell & Worksheet & -- & StudentRecords & -- & D \\\hline 
  12 & 2019-03-03T19:07:55 & Paste & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline 
  13 & 2019-03-03T19:08:02 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline
  14 & 2019-03-03T19:08:05 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Student status & -- \\\hline   
  \rowcolor{red}  
  15 & 2019-03-03T19:08:08 & Click button & Web browser & http://www.unimelb.edu.au & -- & Submit & -- \\\hline
  \rowcolor{green}
  16 & 2019-03-03T19:08:12 & Click button & Web browser & http://www.unimelb.edu.au & -- & New Record & -- \\\hline
  17 & 2019-03-03T19:08:17 & Copy cell & Worskheet & -- & StudentRecords & -- & B \\\hline  
  18 & 2019-03-03T19:08:21 & Paste & Web browser & http://www.unimelb.edu.au & -- & Date & -- \\\hline 
  19 & 2019-03-03T19:08:28 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Date & -- \\\hline
  20 & 2019-03-03T19:08:35 & Copy cell & Worksheet & -- & StudentRecords & -- & C \\\hline 
  21 & 2019-03-03T19:08:38 & Paste & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline 
  22 & 2019-03-03T19:08:39 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline
  23 & 2019-03-03T19:08:40 & Copy cell & Worksheet & -- & StudentRecords & -- & A \\\hline 
  24 & 2019-03-03T19:08:42 & Paste & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline 
  25 & 2019-03-03T19:08:43 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline
  26 & 2019-03-03T19:08:45 & Copy cell & Worksheet & -- & StudentRecords & -- & D \\\hline 
  27 & 2019-03-03T19:08:47 & Paste & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline 
  28 & 2019-03-03T19:08:49 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline
  29 & 2019-03-03T19:08:52 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Student status & -- \\\hline   
  \rowcolor{red}
  30 & 2019-03-03T19:08:53 & Click button & Web browser & http://www.unimelb.edu.au & -- & Submit & -- \\\hline
 \end{tabular}
    }}}
   \caption{Segments identification}\label{tab:segments}
   \vspace{-2mm}
\end{table}
\endgroup




==> tables-complete-uiLog-compact-backup.tex <==
\begingroup
%\renewcommand{\arraystretch}{1.6}
\begin{table}[hbtp]
\makebox[0.98\textwidth][c]{
\centering
{\tiny{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    & \textbf{UI}
    & \textbf{UI}
    & \multicolumn{6}{|c}{\textbf{Payload}}
    \\\cline{4-9}
	
	\textbf{Row}
    & \textbf{Timestamp}
    & \textbf{Type}
    & $\boldmath{P_1}$
    & $\boldmath{P_2}$
    & $\boldmath{P_3}$
    & $\boldmath{P_4}$
    & $\boldmath{P_5}$
    & $\boldmath{P_6}$\\\hline

    1 & 2019-03-03T19:02:18 & Click button (Web) & https://unimelb.edu.au & New Record & newRecord & button & -- & --  \\\hline
    2 & 2019-03-03T19:02:23 & Copy cell (Excel) & StudentRecords & Sheet1 & A & 2 & Albert Rauf & Albert Rauf \\\hline 
    3 & 2019-03-03T19:02:26 & Paste (Web) & https://unimelb.edu.au & Full Name & name & ``'' & Albert Rauf & -- \\\hline 
    4 & 2019-03-03T19:02:28 & Edit field (Web) & https://unimelb.edu.au & Full Name & name & text & Albert Rauf & -- \\\hline
    5 & 2019-03-03T19:02:31 & Copy cell (Excel) & StudentRecords & Sheet1 & B & 2 & 11/04/1986 & 11/04/1986 \\\hline  
    6 & 2019-03-03T19:02:37 & Paste (Web) & https://unimelb.edu.au & Date & date & ``'' & 11/04/1986 & -- \\\hline 
    7 & 2019-03-03T19:02:40 & Edit field (Web) &  https://unimelb.edu.au & Date & date & text & 11-04-1986 & --  \\\hline
    8 & 2019-03-03T19:07:33 & Copy cell (Excel) & StudentRecords & Sheet1 & C & 2 & +61 043 512 4834 & +61 043 512 4834 \\\hline 
    9 & 2019-03-03T19:07:40 & Paste (Web) & https://unimelb.edu.au & Phone & phone & ``'' & +61 043 512 4834 & -- \\\hline 
  10 & 2019-03-03T19:07:48 & Edit field (Web) & https://unimelb.edu.au & Phone & phone & text & 043-512-4834 & -- \\\hline
  11 & 2019-03-03T19:07:50 & Copy cell (Excel) & StudentRecords & Sheet1 & D & 2 & Germany & Germany \\\hline 
  12 & 2019-03-03T19:07:55 & Paste (Web) & https://unimelb.edu.au & Country of residence & country & ``'' & Germany & -- \\\hline 
  13 & 2019-03-03T19:08:02 & Edit field (Web) & https://unimelb.edu.au & Country of residence & country & text & Germany & --  \\\hline
  14 & 2019-03-03T19:08:05 & Edit field (Web) & https://unimelb.edu.au & Student status & status & select & International & -- \\\hline   
  15 & 2019-03-03T19:08:08 & Click button (Web) & https://unimelb.edu.au & Submit & submit & submit & -- & --\\\hline
  16 & 2019-03-03T19:08:12 & Click button (Web) & https://unimelb.edu.au & New Record & newRecord & button & -- & -- \\\hline
  17 & 2019-03-03T19:08:17 & Copy cell (Excel) & StudentRecords & Sheet1 & B & 3 & 20/06/1987 & 20/06/1987 \\\hline  
  18 & 2019-03-03T19:08:21 & Paste (Web) & https://unimelb.edu.au & Date & date & ``'' & 20/06/1987 & -- \\\hline 
  19 & 2019-03-03T19:08:28 & Edit field (Web) & https://unimelb.edu.au & Date & date & text & 20-06-1987 & -- \\\hline
  20 & 2019-03-03T19:08:35 & Copy cell (Excel) & StudentRecords &  Sheet1 & C & 3 & +61 519 790 1066 & +61 519 790 1066 \\\hline 
  21 & 2019-03-03T19:08:38 & Paste (Web) & https://unimelb.edu.au & Phone & phone & ``'' & +61 519 790 1066 & -- \\\hline 
  22 & 2019-03-03T19:08:39 & Edit field (Web) & https://unimelb.edu.au & Phone & phone & text & 519-790-1066 & -- \\\hline
  23 & 2019-03-03T19:08:40 & Copy cell (Excel) & StudentRecords & Sheet1 & A & 3 & Audrey Backer & Audrey Backer \\\hline 
  24 & 2019-03-03T19:08:42 & Paste (Web) & https://unimelb.edu.au & Full Name & name & ``'' & Audrey Backer & -- \\\hline 
  25 & 2019-03-03T19:08:43 & Edit field (Web) & https://unimelb.edu.au & Full Name & name & text & Audrey Backer & -- \\\hline
  26 & 2019-03-03T19:08:44 & Copy cell (Excel) & StudentRecords & Sheet1 & D & 2 & Germany & Germany \\\hline 
  27 & 2019-03-03T19:08:45 & Copy cell (Excel) & StudentRecords & Sheet1 & D & 3 & Australia & Australia \\\hline 
  28 & 2019-03-03T19:08:47 & Paste (Web) & https://unimelb.edu.au & Country of residence & country & ``'' & Australia & -- \\\hline 
  29 & 2019-03-03T19:08:49 & Edit field (Web) & https://unimelb.edu.au & Country of residence & country & text & Australia & -- \\\hline
  30 & 2019-03-03T19:08:52 & Edit field (Web) & https://unimelb.edu.au & Student status & status & select & Domestic & -- \\\hline   
  31 & 2019-03-03T19:08:53 & Click button (Web) & https://unimelb.edu.au & Submit & submit & submit & -- & -- \\\hline
  \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\\hline
 \end{tabular}
	}}}
   \caption{Fragment of a user interaction log}\label{tab:uilog}
   \vspace{-2mm}
\end{table}
\endgroup




==> tables-complete-uiLog.tex <==
\begingroup
%\renewcommand{\arraystretch}{1.6}
\begin{table}[hbtp]
\makebox[0.98\textwidth][c]{
\centering
{\tiny{
    \begin{tabular}{c|c|c|l|l|l|l|l|l|l|l}
    & \textbf{UI}
    & \textbf{UI}
    & \multicolumn{8}{|c}{\textbf{Payload}}
    \\\cline{4-11}
	
	\textbf{Row}
    & \textbf{Timestamp}
    & \textbf{Type}
    & \textbf{$P_1$: Application}
    & \textbf{$P_2$: URL}
    & \textbf{$P_3$: Worksheet Name}
    & \textbf{$P_4$: Element Label}
    & \textbf{$P_5$: Cell Column}
    & \textbf{$P_6$: Cell Row}
    & \textbf{$P_7$: Element Value}
    & \textbf{$P_8$: Copied/pasted Content}\\\hline

    1 & 2019-03-03T19:02:18 & Click button & Web browser & https://unimelb.edu.au & -- & New Record & -- & -- & -- & -- \\\hline
    2 & 2019-03-03T19:02:23 & Copy cell & Worksheet & -- & StudentRecords & -- & A & 2 & Albert Rauf & Albert Rauf \\\hline 
    3 & 2019-03-03T19:02:26 & Paste & Web browser & https://unimelb.edu.au & -- & Full Name & -- & -- & ``'' & Albert Rauf \\\hline 
    4 & 2019-03-03T19:02:28 & Edit field & Web browser & https://unimelb.edu.au & -- & Full Name & -- & -- & Albert Rauf & -- \\\hline
    5 & 2019-03-03T19:02:31 & Copy cell & Worskheet & -- & StudentRecords & -- & B & 2 & 11/04/1986 & 11/04/1986 \\\hline  
    6 & 2019-03-03T19:02:37 & Paste & Web browser & https://unimelb.edu.au & -- & Date & -- & -- & ``'' & 11/04/1986 \\\hline 
    7 & 2019-03-03T19:02:40 & Edit field & Web browser &  https://unimelb.edu.au & -- & Date & -- & -- & 11-04-1986 & --  \\\hline
    8 & 2019-03-03T19:07:33 & Copy cell & Worksheet & -- & StudentRecords & -- & C & 2 & +61 043 512 4834 & +61 043 512 4834 \\\hline 
    9 & 2019-03-03T19:07:40 & Paste & Web browser & https://unimelb.edu.au & -- & Phone & -- & -- & ``'' & +61 043 512 4834 \\\hline 
  10 & 2019-03-03T19:07:48 & Edit field & Web browser & https://unimelb.edu.au & -- & Phone & -- & -- & 043-512-4834 & -- \\\hline
  11 & 2019-03-03T19:07:50 & Copy cell & Worksheet & -- &  StudentRecords & -- & D & 2 & Germany & Germany \\\hline 
  12 & 2019-03-03T19:07:55 & Paste & Web browser & https://unimelb.edu.au & -- & Country of residence & -- & -- & ``'' & Germany  \\\hline 
  13 & 2019-03-03T19:08:02 & Edit field & Web browser & https://unimelb.edu.au & -- & Country of residence & -- & -- & Germany & --  \\\hline
  14 & 2019-03-03T19:08:05 & Edit field & Web browser & https://unimelb.edu.au & -- & Student status & -- & -- & International & -- \\\hline   
  15 & 2019-03-03T19:08:08 & Click button & Web browser & https://unimelb.edu.au & -- & Submit & -- & -- & -- & -- \\\hline
  16 & 2019-03-03T19:08:12 & Click button & Web browser & https://unimelb.edu.au & -- & New Record & -- & -- & -- & -- \\\hline
  17 & 2019-03-03T19:08:17 & Copy cell & Worskheet & -- & StudentRecords & -- & B & 3 & 20/06/1987 & 20/06/1987 \\\hline  
  18 & 2019-03-03T19:08:21 & Paste & Web browser & https://unimelb.edu.au & -- & Date & -- & -- & ``'' & 20/06/1987 \\\hline 
  19 & 2019-03-03T19:08:28 & Edit field & Web browser & https://unimelb.edu.au & -- & Date & -- & -- & 20-06-1987 & -- \\\hline
  20 & 2019-03-03T19:08:35 & Copy cell & Worksheet & -- & StudentRecords &  -- & C & 3 & +61 519 790 1066 & +61 519 790 1066 \\\hline 
  21 & 2019-03-03T19:08:38 & Paste & Web browser & https://unimelb.edu.au & -- & Phone & -- & -- & ``'' & +61 519 790 1066 \\\hline 
  22 & 2019-03-03T19:08:39 & Edit field & Web browser & https://unimelb.edu.au & -- & Phone & -- & -- & 519-790-1066 & -- \\\hline
  23 & 2019-03-03T19:08:40 & Copy cell & Worksheet & -- & StudentRecords & -- & A & 3 & Audrey Backer & Audrey Backer \\\hline 
  24 & 2019-03-03T19:08:42 & Paste & Web browser & https://unimelb.edu.au & -- & Full Name & -- & -- & ``'' & Audrey Backer \\\hline 
  25 & 2019-03-03T19:08:43 & Edit field & Web browser & https://unimelb.edu.au & -- & Full Name & -- & -- & Audrey Backer & -- \\\hline
  26 & 2019-03-03T19:08:44 & Copy cell & Worksheet & -- & StudentRecords & -- & D & 2 & Germany & Germany \\\hline 
  27 & 2019-03-03T19:08:45 & Copy cell & Worksheet & -- & StudentRecords & -- & D & 3 & Australia & Australia \\\hline 
  28 & 2019-03-03T19:08:47 & Paste & Web browser & https://unimelb.edu.au & -- & Country of residence & -- & -- & ``'' & Australia \\\hline 
  29 & 2019-03-03T19:08:49 & Edit field & Web browser & https://unimelb.edu.au & -- & Country of residence & -- & -- & Australia & -- \\\hline
  30 & 2019-03-03T19:08:52 & Edit field & Web browser & https://unimelb.edu.au & -- & Student status & -- & -- & Domestic & -- \\\hline   
  31 & 2019-03-03T19:08:53 & Click button & Web browser & https://unimelb.edu.au & -- & Submit & -- & -- & -- & -- \\\hline
  \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\\hline
 \end{tabular}
	}}}
   \caption{Fragment of a user interaction log}\label{tab:uilog}
   \vspace{-2mm}
\end{table}
\endgroup




==> tables-complete-uiLogNorm.tex <==
\begingroup
%\renewcommand{\arraystretch}{1.6}
\begin{table}[hbtp]
\makebox[0.98\textwidth][c]{
\centering
{\tiny{
    \begin{tabular}{c|c|c|l|l|l|l|l}
    & \textbf{UI}
    & \textbf{UI}
    & \multicolumn{5}{|c}{\textbf{Payload}}
    \\\cline{4-8}

    & \textbf{Timestamp}
    & \textbf{Type}
    & \textbf{\textbf{$P_1$: Application}}
    & \textbf{\textbf{$P_2$: URL}}
    & \textbf{\textbf{$P_3$: Worksheet Name}}
    & \textbf{\textbf{$P_4$: Element Label}}
    & \textbf{\textbf{$P_5$: Cell Column}}\\\hline

    1 & 2019-03-03T19:02:18 & Click button & Web browser & http://www.unimelb.edu.au & -- & New Record & -- \\\hline
    2 & 2019-03-03T19:02:23 & Copy cell & Worksheet & -- & StudentRecords & -- & A \\\hline 
    3 & 2019-03-03T19:02:26 & Paste & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline 
    4 & 2019-03-03T19:02:28 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline
    5 & 2019-03-03T19:02:31 & Copy cell & Worskheet & -- & StudentRecords & -- & B \\\hline  
    6 & 2019-03-03T19:02:37 & Paste & Web browser & http://www.unimelb.edu.au & -- & Date & -- \\\hline 
    7 & 2019-03-03T19:02:40 & Edit field & Web browser & http://www.unimelb.edu.au &-- & Date & -- \\\hline
    8 & 2019-03-03T19:07:33 & Copy cell & Worksheet & -- & StudentRecords & -- & C \\\hline 
    9 & 2019-03-03T19:07:40 & Paste & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline 
  10 & 2019-03-03T19:07:48 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline
  11 & 2019-03-03T19:07:50 & Copy cell & Worksheet & -- & StudentRecords & -- & D \\\hline 
  12 & 2019-03-03T19:07:55 & Paste & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline 
  13 & 2019-03-03T19:08:02 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline
  14 & 2019-03-03T19:08:05 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Student status & -- \\\hline   
  15 & 2019-03-03T19:08:08 & Click button & Web browser & http://www.unimelb.edu.au & -- & Submit & -- \\\hline
  16 & 2019-03-03T19:08:12 & Click button & Web browser & http://www.unimelb.edu.au & -- & New Record & -- \\\hline
  17 & 2019-03-03T19:08:17 & Copy cell & Worskheet & -- & StudentRecords & -- & B \\\hline  
  18 & 2019-03-03T19:08:21 & Paste & Web browser & http://www.unimelb.edu.au & -- & Date & -- \\\hline 
  19 & 2019-03-03T19:08:28 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Date & -- \\\hline
  20 & 2019-03-03T19:08:35 & Copy cell & Worksheet & -- & StudentRecords & -- & C \\\hline 
  21 & 2019-03-03T19:08:38 & Paste & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline 
  22 & 2019-03-03T19:08:39 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Phone & -- \\\hline
  23 & 2019-03-03T19:08:40 & Copy cell & Worksheet & -- & StudentRecords & -- & A \\\hline 
  24 & 2019-03-03T19:08:42 & Paste & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline 
  25 & 2019-03-03T19:08:43 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Full Name & -- \\\hline
  26 & 2019-03-03T19:08:45 & Copy cell & Worksheet & -- & StudentRecords & -- & D \\\hline 
  27 & 2019-03-03T19:08:47 & Paste & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline 
  28 & 2019-03-03T19:08:49 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Country of residence & -- \\\hline
  29 & 2019-03-03T19:08:52 & Edit field & Web browser & http://www.unimelb.edu.au & -- & Student status & -- \\\hline   
  30 & 2019-03-03T19:08:53 & Click button & Web browser & http://www.unimelb.edu.au & -- & Submit & -- \\\hline
 \end{tabular}
    }}}
   \caption{Normalized user interaction log}\label{tab:norm-uilog}
   \vspace{-2mm}
\end{table}
\endgroup




==> tables-dependencyExample2.tex <==
\begin{table}[tbh]
%\vspace{-3mm}
\centering
\scalebox{0.85}{
\begin{tabular}{c|c|c|c|c}
\hline
u1.value & u2.value & u3.value & u4.value & Target \\ \hline
John Doe & 11/03/1986 & Australia & jdoe@gmail.com & +61 \\ 
Steven Richards & 18/06/1986 & Australia & srichards@gmail.com & +61 \\ 
Hilda Diggle & 31/07/1993 & New Zealand & hdiggle@gmail.com & +64 \\ 
Lucca Bianchi & 19/10/1998 & Italy & lbianchi@gmail.com & +39 \\ 
Volodymyr Leno & 17/10/1994 & Ukraine & vleno@gmail.com & +380 \\ 
Alex Bradshaw & 06/10/1991 & United Kingdom & abradshaw@gmail.com & +44 \\ 
Ben Stanley & 03/12/1991 & United Kingdom & bstanley@gmail.com & +44 \\ 
Olga Mykolenchuk & 11/04/2000 & Ukraine & omykolenchuk@gmail.com & +380 \\ 
Daniel Brown & 06/04/1994 & New Zealand & dbrown@gmail.com & +64 \\ \hline
\end{tabular}
}
\caption{Example of a dependency table.}
\label{table:dependencyTable}
%\vspace{-4mm}
\end{table}




==> tables-segmentation.tex <==
\begingroup
\renewcommand{\arraystretch}{1.6}
\begin{table}[hbtp]
	\centering
	\scalebox{0.65}{
    \begin{tabular}{c|c|c|l|l}
    & \textbf{UI}
    & \textbf{UI}
    & \multicolumn{2}{|c}{\textbf{UI Parameters and Values}}
    \\\cline{4-5}

    & \textbf{Timestamp}
    & \textbf{Type}
    & \textbf{\textbf{$P_1$: Application}}
    & \textbf{\textbf{$P_2$: Element Label}}\\\hline

    \rowcolor{green}
    1 & 2019-03-03T19:02:18 & Click button &Web & New Record \\\hline
    2 &  2019-03-03T19:02:23 & Edit field &  Web & Full Name \\\hline
    3 & 2019-03-03T19:02:27 & Edit field & Web & Date \\\hline
    4 & 2019-03-03T19:02:39 & Edit field & Web & Phone \\\hline
    \rowcolor{red}
    5 &  2019-03-03T19:02:47 & Click button & Web & Submit \\\hline
    \rowcolor{green}
    6 & 2019-03-03T19:02:58 & Click button & Web & New Record \\\hline
    7 & 2019-03-03T19:03:13 & Edit field & Web & Date \\\hline
    8 & 2019-03-03T19:03:24 & Edit field & Web & Phone \\\hline
    9 & 2019-03-03T19:03:43 & Edit field & Web & Full Name \\\hline
    \rowcolor{red}
    10 & 2019-03-03T19:04:10 & Click button & Web & Submit \\\hline
    \end{tabular}
    }
  	\caption{Segments identification}\label{tab:segments}
  	\vspace{-2mm}
\end{table}
\endgroup




==> tables-uiLog.tex <==
\begingroup
\renewcommand{\arraystretch}{1.6}
\begin{table}[hbtp]
	\centering
	\scalebox{0.65}{
    \begin{tabular}{c|c|c|l|l|l}
    & \textbf{UI}
    & \textbf{UI}
    & \multicolumn{3}{|c}{\textbf{Payload}}
    \\\cline{4-6}

    & \textbf{Timestamp}
    & \textbf{Type}
    & \textbf{\textbf{$P_1$: Application}}
    & \textbf{\textbf{$P_2$: Element Label}}
    & \textbf{\textbf{$P_3$: Element Value}}\\\hline


    1 & 2019-03-03T19:02:18 & Click button & Web & New Record & --\\\hline
    2 &  2019-03-03T19:02:23 & Edit field & Web & Full Name & Albert Rauf \\\hline
    3 & 2019-03-03T19:02:27 & Edit field & Web & Date & 11-04-1986 \\\hline
    4 & 2019-03-03T19:02:39 & Edit field & Web & Phone & + 61 043 512 4834 \\\hline
    5 &  2019-03-03T19:02:47 & Click button & Web & Submit & --\\\hline
    6 & 2019-03-03T19:02:58 & Click button & Web & New Record & --\\\hline
    7 & 2019-03-03T19:03:13 & Edit field & Web & Date & 20-06-1987 \\\hline
    8 & 2019-03-03T19:03:24 & Edit field & Web & Phone & +61 519 790 1066 \\\hline
    9 & 2019-03-03T19:03:43 & Edit field & Web & Full Name & Audrey Backer \\\hline
    10 & 2019-03-03T19:04:10 & Click button & Web & Submit & --\\\hline
    \end{tabular}
    }
  	\caption{Fragment of a user interaction log.}\label{tab:uilog}
  	\vspace{-2mm}
\end{table}
\endgroup




==> tables-uiLogNorm.tex <==
\begingroup
\renewcommand{\arraystretch}{1.6}
\begin{table}[hbtp]
	\centering
	\scalebox{0.65}{
    \begin{tabular}{c|c|c|l|l}
    & \textbf{UI}
    & \textbf{UI}
    & \multicolumn{2}{|c}{\textbf{UI Parameters and Values}}
    \\\cline{4-5}

    & \textbf{Timestamp}
    & \textbf{Type}
    & \textbf{\textbf{$P_1$: Application}}
    & \textbf{\textbf{$P_2$: Element Label}}\\\hline


    1 & 2019-03-03T19:02:18 & Click button &Web & New Record \\\hline
    2 &  2019-03-03T19:02:23 & Edit field &  Web & Full Name \\\hline
    3 & 2019-03-03T19:02:27 & Edit field & Web & Date \\\hline
    4 & 2019-03-03T19:02:39 & Edit field & Web & Phone \\\hline
    5 &  2019-03-03T19:02:47 & Click button & Web & Submit \\\hline
    6 & 2019-03-03T19:02:58 & Click button & Web & New Record \\\hline
    7 & 2019-03-03T19:03:13 & Edit field & Web & Date \\\hline
    8 & 2019-03-03T19:03:24 & Edit field & Web & Phone \\\hline
    9 & 2019-03-03T19:03:43 & Edit field & Web & Full Name \\\hline
    10 & 2019-03-03T19:04:10 & Click button & Web & Submit \\\hline
    \end{tabular}
    }
  	\caption{Normalised user interaction log.}\label{tab:norm-uilog}
  	\vspace{-2mm}
\end{table}
\endgroup



